Doubly Sparse: Sparse Mixture of Sparse Experts for Efficient Softmax Inference

Computations for the softmax function are significantly expensive when the number of output classes is large. In this paper, we present a novel softmax inference speedup method, Doubly Sparse Softmax (DS-Softmax), that leverages sparse mixture of sparse experts to efficiently retrieve top-k classes. Different from most existing methods that require and approximate a fixed softmax, our method is learning-based and can adapt softmax weights for a better inference speedup. In particular, our method learns a two-level hierarchy which divides entire output class space into several partially overlapping experts. Each expert is sparse and only contains a subset of output classes. To find top-k classes, a sparse mixture enables us to find the most probable expert quickly, and the sparse expert enables us to search within a small-scale softmax. We empirically conduct evaluation on several real-world tasks, including neural machine translation, language modeling and image classification, and demonstrate that significant computation reductions can be achieved at no performance loss.

==> content/backup.tex <==
In terms of experiment setup, we leave the task-specific matters for later, here we present details on our model setup. For real tasks, we find it is easier to first pre-train the whole model with conventional softmax, and replace the softmax layer with DS-Softmax and retrain the new layer while keeping others fixed, with Adam \citep{kingma2014adam}. In terms of hyper-parameters setting,  $\lambda_{load}$ and threshold $\gamma$ are fixed as 10 and 0.01. $\lambda_{lasso}$ and $\lambda_{expert}$ share the same value and are tuned using the following strategy: starting with zero and increasing exponentially until it decreases the performance in validation. The reported performance is on an independent testing dataset.



Neural machine translation task is also usually used for softmax speedup evaluation. We use IWSLT English to Vietnamese dataset \citep{Luong-Manning:iwslt15} and evaluate performance by BLEU score \citep{papineni2002bleu} with greedy searching. The BLEU is assessed on the testing dataset. A vanilla softmax model is seq2seq \citep{sutskever2014sequence} and implemented using TensorFlow\footnote{https://github.com/tensorflow/nmt} \citep{abadi2016tensorflow}. The number of output words is 7,709 and the results are shown in Table~\ref{table:nmt_result}, where our method achieves 15.08x speedup (in terms of FLOPs) with similar BLEU score.

\begin{table}[t]
\small
\begin{minipage}{0.46\textwidth}
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Task} & \textbf{Method} & \textbf{Bleu Score} & \textbf{Speedup} \\\hline
\multirow{5}{*}{\thead{IWSLT \\ En-Ve \\ (7,709)}} & Full & 25.2 & - \\\cline{2-4}
& DS-8 & 25.3 & 4.38x \\\cline{2-4}
& DS-16 & 25.1 & 6.08x \\\cline{2-4}
& DS-32 & \textbf{25.4} & 10.69x \\\cline{2-4}
& DS-64 & 25.0 & \textbf{15.08x} \\\hline
\end{tabular}
\caption{Neural machine translation results on IWSLT English to Vietnamese and the vocabulary size is 7,709.}
\label{table:nmt_result}
\end{minipage}
\hspace{0.05\textwidth}
\begin{minipage}{0.45\textwidth}
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Task} & \textbf{Method} & \textbf{Accuracy} & \textbf{Speedup} \\\hline
\multirow{5}{*}{\thead{CASIA \\ (3,740)}} & Full & 90.6 & - \\\cline{2-4}
& DS-8 & \textbf{90.8} & 1.77x \\\cline{2-4}
& DS-16 & 90.2 & 2.82x \\\cline{2-4}
& DS-32 & 89.9 & 4.72x \\\cline{2-4}
& DS-64 & 90.1 & \textbf{6.91x} \\\hline
\end{tabular} 
\caption{Image classification results on CASIA. There are 3,740 different characters inside dataset.}
\label{table:casia}
\end{minipage}
\end{table}


\subsection{Chinese Character Recognition}
We also test on Chinese handwriting character recognition task. We use the offline and special characters filtered CASIA dataset \citep{liu2011casia}. CAISA is a popular Chinese character recognition dataset with around four thousand characters. Unlike language related task, the class distribution is uniform here rather than unbalanced. Two-thirds of the data is chosen for training and rest for testing. Table~\ref{table:casia} shows the results and we can achieve significant (6.91x) speedup (in terms of FLOPs) on this task.

